Document-editing Assistants and Model-based Reinforcement Learning as a Path to Conversational AI

Intelligent assistants that follow commands or answer simple questions, such as Siri and Google search, are among the most economically important applications of AI. Future conversational AI assistants promise even greater capabilities and a better user experience through a deeper understanding of the domain, the user, or the user's purposes. But what domain and what methods are best suited to researching and realizing this promise? In this article we argue for the domain of voice document editing and for the methods of model-based reinforcement learning. The primary advantages of voice document editing are that the domain is tightly scoped and that it provides something for the conversation to be about (the document) that is delimited and fully accessible to the intelligent assistant. The advantages of reinforcement learning in general are that its methods are designed to learn from interaction without explicit instruction and that it formalizes the purposes of the assistant. Model-based reinforcement learning is needed in order to genuinely understand the domain of discourse and thereby work efficiently with the user to achieve their goals. Together, voice document editing and model-based reinforcement learning comprise a promising research direction for achieving conversational AI.

==> refs.tex <==
\begin{thebibliography}{}

\bibitem[\protect\citeauthoryear{Abbeel \bgroup et al\mbox.\egroup
  }{2007}]{abbeel2007application}
Abbeel, P.; Coates, A.; Quigley, M.; and Ng, A.~Y.
\newblock 2007.
\newblock An application of reinforcement learning to aerobatic helicopter
  flight.
\newblock In {\em Proceedings of the 21st Conference on Neural Information
  Processing Systems},  pp. 1--8.

\bibitem[\protect\citeauthoryear{Ades and Swinehart}{1986}]{ades1986voice}
Ades, S., and Swinehart, D.~C.
\newblock 1986.
\newblock Voice annotation and editing in a workstation environment.
\newblock Technical Report CSL-86-3, XEROX Corporation, Palo Alto Research
  Center.

\bibitem[\protect\citeauthoryear{Allen}{1979}]{allen1979plan}
Allen, J.~F.
\newblock 1979.
\newblock A plan-based approach to speech act recognition.
\newblock Technical Report 131/79, University of Toronto, Department of
  Computer Science.

\bibitem[\protect\citeauthoryear{Anderson, Boyle, and
  Reiser}{1985}]{anderson1985intelligent}
Anderson, J.~R.; Boyle, C.~F.; and Reiser, B.~J.
\newblock 1985.
\newblock Intelligent tutoring systems.
\newblock {\em Science} 228(4698):456--462.

\bibitem[\protect\citeauthoryear{Asri, He, and Suleman}{2016}]{Asri_2016}
Asri, L.~E.; He, J.; and Suleman, K.
\newblock 2016.
\newblock {A Sequence-to-Sequence Model for User Simulation in Spoken Dialogue
  Systems}.
\newblock In {\em Interspeech}.
\newblock ISCA.

\bibitem[\protect\citeauthoryear{{Atkeson} and
  {Santamaria}}{1997}]{Atkeson_1997_mbrl}
{Atkeson}, C.~G., and {Santamaria}, J.~C.
\newblock 1997.
\newblock A comparison of direct and model-based reinforcement learning.
\newblock In {\em Proceedings of International Conference on Robotics and
  Automation}, volume~4,  pp. 3557--3564.

\bibitem[\protect\citeauthoryear{Bagnell and
  Schneider}{2001}]{bagnell2001autonomous}
Bagnell, J.~A., and Schneider, J.~G.
\newblock 2001.
\newblock Autonomous helicopter control using reinforcement learning policy
  search methods.
\newblock In {\em Proceedings 2001 ICRA. IEEE International Conference on
  Robotics and Automation (Cat. No. 01CH37164)}, volume~2,  pp. 1615--1620.
\newblock IEEE.

\bibitem[\protect\citeauthoryear{Bapna \bgroup et al\mbox.\egroup
  }{2017}]{bapna2017towards}
Bapna, A.; T{\"u}r, G.; Hakkani-T{\"u}r, D.; and Heck, L.
\newblock 2017.
\newblock Towards zero-shot frame semantic parsing for domain scaling.
\newblock {\em ArXiv:1707.02363}.

\bibitem[\protect\citeauthoryear{Bassiri}{2011}]{bassiri2011interactional}
Bassiri, M.~A.
\newblock 2011.
\newblock {Interactional Feedback and the Impact of Attitude and Motivation on
  Noticing L2 Form}.
\newblock {\em English Language and Literature Studies} 1(2):61.

\bibitem[\protect\citeauthoryear{Berkenkamp \bgroup et al\mbox.\egroup
  }{2017}]{berkenkamp2017safe}
Berkenkamp, F.; Turchetta, M.; Schoellig, A.; and Krause, A.
\newblock 2017.
\newblock Safe model-based reinforcement learning with stability guarantees.
\newblock In {\em Proceedings of the 31st Conference on Neural Information
  Processing Systems},  pp. 908--918.

\bibitem[\protect\citeauthoryear{Biermann and
  Long}{1996}]{biermann1996composition}
Biermann, A.~W., and Long, P.~M.
\newblock 1996.
\newblock The composition of messages in speech-graphics interactive systems.
\newblock In {\em Proceedings of the 1996 International Symposium on Spoken
  Dialogue},  pp. 97--100.

\bibitem[\protect\citeauthoryear{Bijl and Hyde-Thomson}{2001}]{bijl2001speech}
Bijl, D., and Hyde-Thomson, H.
\newblock 2001.
\newblock {\em Speech to text conversion}.
\newblock US Patent 6,173,259. Google Patents.

\bibitem[\protect\citeauthoryear{Bordes, Boureau, and
  Weston}{2017}]{bordes2016learning}
Bordes, A.; Boureau, Y.-L.; and Weston, J.
\newblock 2017.
\newblock Learning end-to-end goal-oriented dialog.
\newblock In {\em Proceedings of the 5th International Conference on Learning
  Representations}.

\bibitem[\protect\citeauthoryear{Bourbakis and
  Kavraki}{2001}]{bourbakis2001intelligent}
Bourbakis, N.~G., and Kavraki, D.
\newblock 2001.
\newblock An intelligent assistant for navigation of visually impaired people.
\newblock In {\em Proceedings 2nd Annual IEEE International Symposium on
  Bioinformatics and Bioengineering (BIBE 2001)},  pp. 230--235.
\newblock IEEE.

\bibitem[\protect\citeauthoryear{Bruce}{1975}]{bruce1975belief}
Bruce, B.
\newblock 1975.
\newblock Belief systems and language understanding.
\newblock {\em Trends in Linguistics. Studies and Monographs} 19:113--160.

\bibitem[\protect\citeauthoryear{Budzianowski \bgroup et al\mbox.\egroup
  }{2017}]{budzianowski2017sub}
Budzianowski, P.; Ultes, S.; Su, P.-H.; Mrk{\v{s}}i{\'c}, N.; Wen, T.-H.;
  Casanueva, I.; Rojas-Barahona, L.; and Ga{\v{s}}i{\'c}, M.
\newblock 2017.
\newblock Sub-domain modelling for dialogue management with hierarchical
  reinforcement learning.
\newblock {\em ArXiv:1706.06210}.

\bibitem[\protect\citeauthoryear{Buesing \bgroup et al\mbox.\egroup
  }{2018}]{buesing2018learning_gen_models}
Buesing, L.; Weber, T.; Racaniere, S.; Eslami, S. M.~A.; Rezende, D.; Reichert,
  D.~P.; Viola, F.; Besse, F.; Gregor, K.; Hassabis, D.; and Wierstra, D.
\newblock 2018.
\newblock Learning and querying fast generative models for reinforcement
  learning.
\newblock {\em ArXiv:1802.03006}.

\bibitem[\protect\citeauthoryear{Carberry}{1989}]{carberry1989plan}
Carberry, S.
\newblock 1989.
\newblock Plan recognition and its use in understanding dialog.
\newblock In {\em User Models in Dialog Systems}. Springer.
\newblock  pp. 133--162.

\bibitem[\protect\citeauthoryear{Carbonell}{1971}]{carbonell1970mixed}
Carbonell, J.~R.
\newblock 1971.
\newblock Mixed-initiative man-computer instructional dialogues.
\newblock Technical report, Cambridge, Bolt Beranek and Newman.

\bibitem[\protect\citeauthoryear{Card, Moran, and
  Newell}{1980}]{card1980computer}
Card, S.~K.; Moran, T.~P.; and Newell, A.
\newblock 1980.
\newblock {Computer text-editing: An information-processing analysis of a
  routine cognitive skill}.
\newblock {\em Cognitive psychology} 12(1):32--74.

\bibitem[\protect\citeauthoryear{Cassell}{2000}]{cassell2000more}
Cassell, J.
\newblock 2000.
\newblock {More than just another pretty face: Embodied conversational
  interface agents}.
\newblock {\em Communications of the ACM} 43(4):70--78.

\bibitem[\protect\citeauthoryear{Chapman and
  Kaelbling}{1991}]{chapman1991input}
Chapman, D., and Kaelbling, L.~P.
\newblock 1991.
\newblock {Input Generalization in Delayed Reinforcement Learning: An Algorithm
  and Performance Comparisons}.
\newblock In {\em Proceedings of the 1991 International Joint Conference on
  Artificial Intelligence}, volume~91,  pp. 726--731.

\bibitem[\protect\citeauthoryear{Chen \bgroup et al\mbox.\egroup
  }{2018}]{chen2018policy}
Chen, L.; Chang, C.; Chen, Z.; Tan, B.; Ga{\v{s}}i{\'c}, M.; and Yu, K.
\newblock 2018.
\newblock Policy adaptation for deep reinforcement learning-based dialogue
  management.
\newblock In {\em IEEE International Conference on Acoustics, Speech and Signal
  Processing},  pp. 6074--6078.
\newblock IEEE.

\bibitem[\protect\citeauthoryear{Chua \bgroup et al\mbox.\egroup
  }{2018}]{chua2018deep}
Chua, K.; Calandra, R.; McAllister, R.; and Levine, S.
\newblock 2018.
\newblock Deep reinforcement learning in a handful of trials using
  probabilistic dynamics models.
\newblock In {\em Proceedings of the 31st Conference on Neural Information
  Processing Systems},  pp. 4754--4765.

\bibitem[\protect\citeauthoryear{Coates, Abbeel, and Ng}{2017}]{Coates2017}
Coates, A.; Abbeel, P.; and Ng, A.~Y.
\newblock 2017.
\newblock {\em Autonomous Helicopter Flight Using Reinforcement Learning}.
\newblock Boston, MA: Springer US.
\newblock  pp. 75--85.

\bibitem[\protect\citeauthoryear{Cohen}{1978}]{cohen1978knowing}
Cohen, P.~R.
\newblock 1978.
\newblock {\em On Knowing What to Say: Planning Speech Acts}.
\newblock Ph.D. Dissertation, University of Toronto, Department of Computer
  Science.

\bibitem[\protect\citeauthoryear{Croft, Metzler, and
  Strohman}{2010}]{croft2010search}
Croft, W.~B.; Metzler, D.; and Strohman, T.
\newblock 2010.
\newblock {\em Search engines: Information retrieval in practice}, volume 520.
\newblock Addison-Wesley Reading.

\bibitem[\protect\citeauthoryear{Cuay{\'a}huitl \bgroup et al\mbox.\egroup
  }{2005}]{cuayahuitl2005human}
Cuay{\'a}huitl, H.; Renals, S.; Lemon, O.; and Shimodaira, H.
\newblock 2005.
\newblock {Human-computer dialogue simulation using hidden Markov models}.
\newblock In {\em Workshop on Automatic Speech Recognition and Understanding,
  IEEE},  pp. 290--295.
\newblock IEEE.

\bibitem[\protect\citeauthoryear{Cuay{\'a}huitl \bgroup et al\mbox.\egroup
  }{2016}]{cuayahuitl2016deep}
Cuay{\'a}huitl, H.; Yu, S.; Williamson, A.; and Carse, J.
\newblock 2016.
\newblock Deep reinforcement learning for multi-domain dialogue systems.
\newblock In {\em Workshop on Deep Reinforcement Learning, NIPS}.

\bibitem[\protect\citeauthoryear{Cuay{\'a}huitl \bgroup et al\mbox.\egroup
  }{2017}]{cuayahuitl2017scaling}
Cuay{\'a}huitl, H.; Yu, S.; Williamson, A.; and Carse, J.
\newblock 2017.
\newblock Scaling up deep reinforcement learning for multi-domain dialogue
  systems.
\newblock In {\em 2017 International Joint Conference on Neural Networks},  pp.
  3339--3346.
\newblock IEEE.

\bibitem[\protect\citeauthoryear{Dario \bgroup et al\mbox.\egroup
  }{1996}]{dario1996robot}
Dario, P.; Guglielmelli, E.; Genovese, V.; and Toro, M.
\newblock 1996.
\newblock {Robot assistants: Applications and evolution}.
\newblock {\em Robotics and autonomous systems} 18(1-2):225--234.

\bibitem[\protect\citeauthoryear{Dean}{2019}]{dean_2019}
Dean, J.
\newblock 2019.
\newblock Looking {B}ack at {G}oogle's {R}esearch {E}fforts in 2018.

\bibitem[\protect\citeauthoryear{Deisenroth and
  Rasmussen}{2011}]{deisenroth2011pilco}
Deisenroth, M., and Rasmussen, C.~E.
\newblock 2011.
\newblock {PILCO: A model-based and data-efficient approach to policy search}.
\newblock In {\em Proceedings of the 28th International Conference on machine
  learning},  pp. 465--472.
\newblock Omnipress.

\bibitem[\protect\citeauthoryear{Deisenroth, Fox, and
  Rasmussen}{2013}]{deisenroth2013gaussian}
Deisenroth, M.~P.; Fox, D.; and Rasmussen, C.~E.
\newblock 2013.
\newblock Gaussian processes for data-efficient learning in robotics and
  control.
\newblock {\em IEEE transactions on pattern analysis and machine intelligence}
  37(2):pp. 408--423.

\bibitem[\protect\citeauthoryear{Dhingra \bgroup et al\mbox.\egroup
  }{2017}]{dhingra2016towards}
Dhingra, B.; Li, L.; Li, X.; Gao, J.; Chen, Y.-N.; Ahmed, F.; and Deng, L.
\newblock 2017.
\newblock Towards end-to-end reinforcement learning of dialogue agents for
  information access.
\newblock In {\em Proceedings of the 55th Annual Meeting of the Association for
  Computational Linguistics},  pp. 484--495.

\bibitem[\protect\citeauthoryear{Doll, Simon, and Daw}{2012}]{doll2012ubiquity}
Doll, B.~B.; Simon, D.~A.; and Daw, N.~D.
\newblock 2012.
\newblock The ubiquity of model-based reinforcement learning.
\newblock {\em Current opinion in neurobiology} 22(6):1075--1081.

\bibitem[\protect\citeauthoryear{Douglas}{1999}]{douglas1999method}
Douglas, H.~R.
\newblock 1999.
\newblock {\em Method and apparatus for editing documents through voice
  recognition}.
\newblock US Patent 5,875,429, Google Patents.

\bibitem[\protect\citeauthoryear{Duffy}{2018}]{duffy}
Duffy, J.
\newblock 2018.
\newblock {\em {The Best Dictation Software for 2019}}.
\newblock {https://zapier.com/blog/best-text-dictation-software} [Accessed July
  27, 2020].

\bibitem[\protect\citeauthoryear{Engelbart}{1962}]{engelbart1962augmenting}
Engelbart, D.~C.
\newblock 1962.
\newblock Augmenting human intellect: A conceptual framework.
\newblock Technical Report AFOSR-3223, Stanford Research Institute.

\bibitem[\protect\citeauthoryear{Eric}{2020}]{Mihail2019convAIrecap}
Eric, M.
\newblock 2020.
\newblock {NeurIPS 2019 ConvAI Workshop Recap}.
\newblock {\em IEEE Signal Processing Society}.
\newblock {https://openai.com/blog/better-language-models} [Accessed July 27,
  2020].

\bibitem[\protect\citeauthoryear{Fain and Pedersen}{2006}]{fain2006sponsored}
Fain, D.~C., and Pedersen, J.~O.
\newblock 2006.
\newblock Sponsored search: A brief history.
\newblock {\em Bulletin of the American Society for Information Science and
  Technology} 32(2):12--13.

\bibitem[\protect\citeauthoryear{Fazel-Zarandi \bgroup et al\mbox.\egroup
  }{2017}]{fazel2017learning}
Fazel-Zarandi, M.; Li, S.-W.; Cao, J.; Casale, J.; Henderson, P.; Whitney, D.;
  and Geramifard, A.
\newblock 2017.
\newblock Learning robust dialog policies in noisy environments.
\newblock In {\em 1st Workshop on Conversational AI, NIPS}.

\bibitem[\protect\citeauthoryear{Feng \bgroup et al\mbox.\egroup
  }{2019}]{feng2019docdial}
Feng, S.; Fadni, K.; Liao, Q.~V.; and Lastras, L.~A.
\newblock 2019.
\newblock {Doc2Dial: A Framework for Dialogue Composition Grounded in Business
  Documents}.
\newblock In {\em Workshop on Document Intelligence, NeurIPS}.

\bibitem[\protect\citeauthoryear{Ferreira and
  Lefèvre}{2015}]{Ferreira2015_online}
Ferreira, E., and Lefèvre, F.
\newblock 2015.
\newblock Reinforcement-learning based dialogue system for human–robot
  interactions with socially-inspired rewards.
\newblock {\em Computer Speech & Language} 34(1):256--274.

\bibitem[\protect\citeauthoryear{Finin, Joshi, and
  Webber}{1986}]{finin1986natural}
Finin, T.~W.; Joshi, A.~K.; and Webber, B.~L.
\newblock 1986.
\newblock Natural language interactions with artificial experts.
\newblock {\em Proceedings of the IEEE} 74(7):921--938.

\bibitem[\protect\citeauthoryear{Finn, Abbeel, and
  Levine}{2017}]{finn2017model}
Finn, C.; Abbeel, P.; and Levine, S.
\newblock 2017.
\newblock Model-agnostic meta-learning for fast adaptation of deep networks.
\newblock In {\em Proceedings of the 34th International Conference on Machine
  Learning-Volume 70},  pp. 1126--1135.
\newblock JMLR.org.

\bibitem[\protect\citeauthoryear{Foerster \bgroup et al\mbox.\egroup
  }{2016}]{foerster2016learning}
Foerster, J.; Assael, I.~A.; De~Freitas, N.; and Whiteson, S.
\newblock 2016.
\newblock Learning to communicate with deep multi-agent reinforcement learning.
\newblock In {\em Proceedings of the 30th Conference on Advances in Neural
  Information Processing Systems},  pp. 2137--2145.

\bibitem[\protect\citeauthoryear{Forrester}{1971}]{forrester1971counterintuitive}
Forrester, J.~W.
\newblock 1971.
\newblock Counterintuitive behavior of social systems.
\newblock {\em Theory and decision} 2(2):pp. 109--140.

\bibitem[\protect\citeauthoryear{Fox and Smith}{1984}]{fox1984isis}
Fox, M.~S., and Smith, S.~F.
\newblock 1984.
\newblock Isis—a knowledge-based system for factory scheduling.
\newblock {\em Expert systems} 1(1):25--49.

\bibitem[\protect\citeauthoryear{Freeman, Ha, and
  Metz}{2019}]{freeman2019learning}
Freeman, D.; Ha, D.; and Metz, L.
\newblock 2019.
\newblock {Learning to Predict Without Looking Ahead: World Models Without
  Forward Prediction}.
\newblock In {\em Proceedings of the 33rd Conference on Advances in Neural
  Information Processing Systems},  pp. 5380--5391.

\bibitem[\protect\citeauthoryear{Gao \bgroup et al\mbox.\egroup
  }{2019}]{gao2019neural}
Gao, J.; Galley, M.; Li, L.; et~al.
\newblock 2019.
\newblock {Neural Approaches to Conversational AI}.
\newblock In {\em Foundations and Trends{\textregistered} in Information
  Retrieval}, volume~13,  pp. 127--298.
\newblock Now Publishers, Inc.

\bibitem[\protect\citeauthoryear{Ga{\v{s}}i{\'c} \bgroup et al\mbox.\egroup
  }{2011}]{gavsic2011line}
Ga{\v{s}}i{\'c}, M.; Jur{\v{c}}{\'\i}{\v{c}}ek, F.; Thomson, B.; Yu, K.; and
  Young, S.
\newblock 2011.
\newblock On-line policy optimisation of spoken dialogue systems via live
  interaction with human subjects.
\newblock In {\em IEEE Workshop on Automatic Speech Recognition \&
  Understanding},  pp. 312--317.
\newblock IEEE.

\bibitem[\protect\citeauthoryear{Ga{\v{s}}i{\'c} \bgroup et al\mbox.\egroup
  }{2013a}]{gavsic2013line}
Ga{\v{s}}i{\'c}, M.; Breslin, C.; Henderson, M.; Kim, D.; Szummer, M.; Thomson,
  B.; Tsiakoulis, P.; and Young, S.
\newblock 2013a.
\newblock On-line policy optimisation of bayesian spoken dialogue systems via
  human interaction.
\newblock In {\em 2013 IEEE International Conference on Acoustics, Speech and
  Signal Processing},  pp. 8367--8371.
\newblock IEEE.

\bibitem[\protect\citeauthoryear{Ga{\v{s}}i{\'c} \bgroup et al\mbox.\egroup
  }{2013b}]{gasic-2013-pomdp}
Ga{\v{s}}i{\'c}, M.; Breslin, C.; Henderson, M.; Kim, D.; Szummer, M.; Thomson,
  B.; Tsiakoulis, P.; and Young, S.
\newblock 2013b.
\newblock {POMDP}-based dialogue manager adaptation to extended domains.
\newblock In {\em Proceedings of the {SIGDIAL} 2013 Conference},  pp. 214--222.
\newblock Metz, France: Association for Computational Linguistics.

\bibitem[\protect\citeauthoryear{Ga{\v{s}}i{\'c} \bgroup et al\mbox.\egroup
  }{2017}]{gavsic2017dialogue}
Ga{\v{s}}i{\'c}, M.; Mrk{\v{s}}i{\'c}, N.; Rojas-Barahona, L.~M.; Su, P.-H.;
  Ultes, S.; Vandyke, D.; Wen, T.-H.; and Young, S.
\newblock 2017.
\newblock Dialogue manager domain adaptation using gaussian process
  reinforcement learning.
\newblock {\em Computer Speech \& Language} 45:552--569.

\bibitem[\protect\citeauthoryear{Gass and Varonis}{1994}]{gass_varonis_1994}
Gass, S.~M., and Varonis, E.~M.
\newblock 1994.
\newblock Input, interaction, and second language production.
\newblock {\em Studies in Second Language Acquisition} 16(3):283--302.

\bibitem[\protect\citeauthoryear{{Google AI Blog. Digital
  Inspiration}}{2020}]{dictationIO}
{Google AI Blog. Digital Inspiration}.
\newblock 2020.
\newblock {\em Dictation.io}.
\newblock {http://dictation.io} [Accessed July 27, 2020].

\bibitem[\protect\citeauthoryear{{Google}}{2020}]{googleDoc}
{Google}.
\newblock 2020.
\newblock {\em {Type with your voice: Edit your document}}.
\newblock {https://support.google.com/docs/answer/4492226} [Accessed February
  22, 2020].

\bibitem[\protect\citeauthoryear{Goyal, Niekum, and
  Mooney}{2019}]{goyal2019using}
Goyal, P.; Niekum, S.; and Mooney, R.~J.
\newblock 2019.
\newblock Using natural language for reward shaping in reinforcement learning.
\newblock In Kraus, S., ed., {\em Proceedings of the Twenty-Eighth
  International Joint Conference on Artificial Intelligence},  pp. 2385--2391.
\newblock Macao, China: International Joint Conferences on Artificial
  Intelligence Organization.

\bibitem[\protect\citeauthoryear{Greyson \bgroup et al\mbox.\egroup
  }{1997}]{greyson1997method}
Greyson, A.~M.; Hokit, J.~D.; Kaptanoglu, M.; Wagner, A.~M.; and Capps, S.~P.
\newblock 1997.
\newblock {\em Method and apparatus for the manipulation of text on a computer
  display screen}.
\newblock US Patent 5,666,552. Google Patents.

\bibitem[\protect\citeauthoryear{Griffith \bgroup et al\mbox.\egroup
  }{2013}]{griffith2013policy}
Griffith, S.; Subramanian, K.; Scholz, J.; Isbell, C.~L.; and Thomaz, A.~L.
\newblock 2013.
\newblock Policy shaping: Integrating human feedback with reinforcement
  learning.
\newblock In {\em Proceedings of the 27th Conference on Advances in Neural
  Information Processing Systems},  pp. 2625--2633.

\bibitem[\protect\citeauthoryear{Grignetti, Hausmann, and
  Gould}{1975}]{grignetti1975intelligent}
Grignetti, M.~C.; Hausmann, C.; and Gould, L.
\newblock 1975.
\newblock An intelligent on-line assistant and tutor: {NLS-SCHOLAR}.
\newblock In {\em Proceedings of the May 19-22, 1975, National Computer
  Conference and Exposition},  pp. 775--781.
\newblock ACM.

\bibitem[\protect\citeauthoryear{Grosz}{1983}]{grosz1983team}
Grosz, B.
\newblock 1983.
\newblock Team: A transportable natural language interface system.
\newblock In {\em Proceedings of the 1st Conference on Applied Natural Language
  Processing},  pp. 38--45.
\newblock Santa Monica, California: Association for Computational Linguistics.

\bibitem[\protect\citeauthoryear{Gruber and Clark}{2017}]{gruber2017dictation}
Gruber, T.~R., and Clark, G.~C.
\newblock 2017.
\newblock {\em Dictation that allows editing}.
\newblock US Patent App. 15/268,215. Google Patents.

\bibitem[\protect\citeauthoryear{Gu \bgroup et al\mbox.\egroup
  }{2019}]{gu2019dialogwae}
Gu, X.; Cho, K.; Ha, J.-W.; and Kim, S.
\newblock 2019.
\newblock Dialog{WAE}: Multimodal response generation with conditional
  wasserstein auto-encoder.
\newblock In {\em International Conference on Learning Representations}.

\bibitem[\protect\citeauthoryear{Gupta \bgroup et al\mbox.\egroup
  }{2019}]{gupta2019casanlu}
Gupta, A.; Zhang, P.; Lalwani, G.; and Diab, M.
\newblock 2019.
\newblock {CASA-NLU}: Context-{A}ware {S}elf-{A}ttentive {N}atural {L}anguage
  {U}nderstanding for {T}ask-oriented {C}hatbots.
\newblock In {\em Proceedings of EMNLP-IJCNLP 2019}.

\bibitem[\protect\citeauthoryear{Ha and Schmidhuber}{2018}]{ha2018world}
Ha, D., and Schmidhuber, J.
\newblock 2018.
\newblock World models.
\newblock In {\em Proceedings of the Thirty-second Conference on Neural
  Information Processing Systems}.
\newblock Montr{\'e}al, Canada: Curran Associates, Inc.

\bibitem[\protect\citeauthoryear{Hafner \bgroup et al\mbox.\egroup
  }{2018}]{hafner2018learning}
Hafner, D.; Lillicrap, T.; Fischer, I.; Villegas, R.; Ha, D.; Lee, H.; and
  Davidson, J.
\newblock 2018.
\newblock Learning latent dynamics for planning from pixels.
\newblock In {\em Proceedings of the 36th International Conference on Machine
  Learning}.
\newblock Long Beach, USA: PMLR.

\bibitem[\protect\citeauthoryear{Hawkins}{1968}]{hawkins1968nature}
Hawkins, D.
\newblock 1968.
\newblock The nature of purpose.
\newblock In {\em Purposive systems: Proceedings of the first annual symposium
  of the American Society for Cybernetics},  pp. 163--173.

\bibitem[\protect\citeauthoryear{He \bgroup et al\mbox.\egroup
  }{2015}]{he2015deep}
He, J.; Chen, J.; He, X.; Gao, J.; Li, L.; Deng, L.; and Ostendorf, M.
\newblock 2015.
\newblock Deep reinforcement learning with a natural language action space.
\newblock {\em ArXiv:1511.04636}.

\bibitem[\protect\citeauthoryear{Hernandaz and
  Arkun}{1990}]{hernandaz1990neural}
Hernandaz, E., and Arkun, Y.
\newblock 1990.
\newblock Neural network modeling and an extended dmc algorithm to control
  nonlinear systems.
\newblock In {\em 1990 American Control Conference},  pp. 2454--2459.
\newblock IEEE.

\bibitem[\protect\citeauthoryear{Higashinaka \bgroup et al\mbox.\egroup
  }{2014}]{higashinaka2014towards}
Higashinaka, R.; Imamura, K.; Meguro, T.; Miyazaki, C.; Kobayashi, N.;
  Sugiyama, H.; Hirano, T.; Makino, T.; and Matsuo, Y.
\newblock 2014.
\newblock Towards an open-domain conversational system fully based on natural
  language processing.
\newblock In {\em Proceedings of COLING 2014, the 25th International Conference
  on Computational Linguistics: Technical Papers},  pp. 928--939.

\bibitem[\protect\citeauthoryear{Holland, Talvitie, and
  Bowling}{2018}]{holland2018effect}
Holland, G.~Z.; Talvitie, E.~J.; and Bowling, M.
\newblock 2018.
\newblock {The Effect of Planning Shape on Dyna-style Planning in
  High-dimensional State Spaces}.
\newblock {\em ArXiv:1806.01825}.

\bibitem[\protect\citeauthoryear{Hoy}{2018}]{hoy2018alexa}
Hoy, M.~B.
\newblock 2018.
\newblock Alexa, {S}iri, {C}ortana, and more: an introduction to voice
  assistants.
\newblock {\em Medical reference services quarterly} 37(1):81--88.

\bibitem[\protect\citeauthoryear{Huang, Zhu, and
  Gao}{2020}]{huang2020challenges}
Huang, M.; Zhu, X.; and Gao, J.
\newblock 2020.
\newblock Challenges in building intelligent open-domain dialog systems.
\newblock {\em ACM Transactions on Information Systems (TOIS)} 38(3):1--32.

\bibitem[\protect\citeauthoryear{Jang, Lee, and Kim}{2019}]{jang2019bayes}
Jang, Y.; Lee, J.; and Kim, K.-E.
\newblock 2019.
\newblock {Bayes-Adaptive Monte-Carlo Planning and Learning for Goal-Oriented
  Dialogues}.
\newblock In {\em 3rd Workshop on Conversational AI, NeurIPS}.
\newblock Vancouver, Canada: Neural Information Processing Systems.

\bibitem[\protect\citeauthoryear{Jaques \bgroup et al\mbox.\egroup
  }{2019}]{jaques2019way}
Jaques, N.; Ghandeharioun, A.; Shen, J.~H.; Ferguson, C.; Lapedriza, A.; Jones,
  N.; Gu, S.; and Picard, R.
\newblock 2019.
\newblock Way off-policy batch deep reinforcement learning of implicit human
  preferences in dialog.
\newblock {\em ArXiv:1907.00456}.

\bibitem[\protect\citeauthoryear{Jiang \bgroup et al\mbox.\egroup
  }{2015}]{jiang2015automatic}
Jiang, J.; Hassan~Awadallah, A.; Jones, R.; Ozertem, U.; Zitouni, I.;
  Gurunath~Kulkarni, R.; and Khan, O.~Z.
\newblock 2015.
\newblock {Automatic Online Evaluation of Intelligent Assistants}.
\newblock In {\em Proceedings of the 24th International Conference on World
  Wide Web},  pp. 506--516.

\bibitem[\protect\citeauthoryear{Jiang \bgroup et al\mbox.\egroup
  }{2019}]{Jiang_2019_planning}
Jiang, Z.; Mao, X.-L.; Huang, Z.; Ma, J.; and Li, S.
\newblock 2019.
\newblock {Towards End-to-End Learning for Efficient Dialogue Agent by Modeling
  Looking-ahead Ability}.
\newblock {\em Proceedings of the 20th Annual SIGdial Meeting on Discourse and
  Dialogue}.

\bibitem[\protect\citeauthoryear{Kaiser \bgroup et al\mbox.\egroup
  }{2019}]{kaiser2019_SimPle_model}
Kaiser, L.; Babaeizadeh, M.; Milos, P.; Osinski, B.; Campbell, R.~H.;
  Czechowski, K.; Erhan, D.; Finn, C.; Kozakowski, P.; Levine, S.; Mohiuddin,
  A.; Sepassi, R.; Tucker, G.; and Michalewski, H.
\newblock 2019.
\newblock {Model-based reinforcement learning for Atari}.
\newblock {\em ArXiv:1903.00374}.

\bibitem[\protect\citeauthoryear{Kaiser, Feiler, and
  Popovich}{1988}]{kaiser1988intelligent}
Kaiser, G.~E.; Feiler, P.~H.; and Popovich, S.~S.
\newblock 1988.
\newblock Intelligent assistance for software development and maintenance.
\newblock {\em IEEE software} 5(3):40--49.

\bibitem[\protect\citeauthoryear{Kamm}{1995}]{kamm1995user}
Kamm, C.
\newblock 1995.
\newblock User interfaces for voice applications.
\newblock In {\em Proceedings of the National Academy of Sciences}, volume~92,
  pp. 10031--10037.
\newblock National Acad Sciences.

\bibitem[\protect\citeauthoryear{Kamthe and
  Deisenroth}{2018}]{kamthe2018data_eff}
Kamthe, S., and Deisenroth, M.
\newblock 2018.
\newblock Data-efficient reinforcement learning with probabilistic model
  predictive control.
\newblock In Storkey, A., and Perez-Cruz, F., eds., {\em Proceedings of the
  21st International Conference on Artificial Intelligence and Statistics},
  volume~84 of {\em Proceedings of Machine Learning Research},  pp. 1701--1710.
\newblock Lanzarote, Spain: PMLR.

\bibitem[\protect\citeauthoryear{Kaplan \bgroup et al\mbox.\egroup
  }{2002}]{kaplan2002robotic}
Kaplan, F.; Oudeyer, P.-Y.; Kubinyi, E.; and Mikl{\'o}si, A.
\newblock 2002.
\newblock Robotic clicker training.
\newblock {\em Robotics and Autonomous Systems} 38(3-4):197--206.

\bibitem[\protect\citeauthoryear{Kaplan, Sauer, and
  Sosa}{2017}]{kaplan2017beating}
Kaplan, R.; Sauer, C.; and Sosa, A.
\newblock 2017.
\newblock Beating {A}tari with natural language guided reinforcement learning.
\newblock {\em ArXiv:1704.05539}.

\bibitem[\protect\citeauthoryear{Knox and Stone}{2012}]{knox2012reinforcement}
Knox, W.~B., and Stone, P.
\newblock 2012.
\newblock Reinforcement learning from simultaneous human and {MDP} reward.
\newblock In {\em Proceedings of the 11th International Conference on
  Autonomous Agents and Multiagent Systems-Volume 1},  pp. 475--482.
\newblock International Foundation for Autonomous Agents and Multiagent
  Systems.

\bibitem[\protect\citeauthoryear{Kocijan \bgroup et al\mbox.\egroup
  }{2004}]{kocijan2004gaussian}
Kocijan, J.; Murray-Smith, R.; Rasmussen, C.~E.; and Girard, A.
\newblock 2004.
\newblock Gaussian process model based predictive control.
\newblock In {\em Proceedings of the 2004 American control conference},
  volume~3,  pp. 2214--2219.
\newblock IEEE.

\bibitem[\protect\citeauthoryear{Kozierok and
  Maes}{1993}]{kozierok1993learning}
Kozierok, R., and Maes, P.
\newblock 1993.
\newblock A learning interface agent for scheduling meetings.
\newblock In {\em Proceedings of the 1st international conference on
  Intelligent user interfaces},  pp. 81--88.
\newblock ACM.

\bibitem[\protect\citeauthoryear{Kudashkina \bgroup et al\mbox.\egroup
  }{2020}]{kudashkina2020sampleefficient}
Kudashkina, K.; Chockalingam, V.; Taylor, G.~W.; and Bowling, M.
\newblock 2020.
\newblock {Sample-Efficient Model-based Actor-Critic for an Interactive
  Dialogue Task}.
\newblock {\em ArXiv:2004.13657}.

\bibitem[\protect\citeauthoryear{Lau \bgroup et al\mbox.\egroup
  }{2001}]{lau2001learning}
Lau, T.; Wolfman, S.~A.; Domingos, P.; and Weld, D.~S.
\newblock 2001.
\newblock {Learning repetitive text-editing procedures with SMARTedit}.
\newblock In {\em Your wish is my command}. Elsevier.
\newblock  pp. 209--XI.

\bibitem[\protect\citeauthoryear{Lazaridou, Pham, and
  Baroni}{2016}]{lazaridou2016towards}
Lazaridou, A.; Pham, N.~T.; and Baroni, M.
\newblock 2016.
\newblock Towards multi-agent communication-based language learning.
\newblock {\em ArXiv:1605.07133}.

\bibitem[\protect\citeauthoryear{Levin, Pieraccini, and
  Eckert}{1997}]{levin1997learning}
Levin, E.; Pieraccini, R.; and Eckert, W.
\newblock 1997.
\newblock Learning dialogue strategies within the {M}arkov decision process
  framework.
\newblock In {\em IEEE Workshop on Automatic Speech Recognition and
  Understanding Proceedings},  pp. 72--79.
\newblock IEEE.

\bibitem[\protect\citeauthoryear{Levine and Abbeel}{2014}]{levine2014learning}
Levine, S., and Abbeel, P.
\newblock 2014.
\newblock Learning neural network policies with guided policy search under
  unknown dynamics.
\newblock In {\em Advances in Neural Information Processing Systems},  pp.
  1071--1079.
\newblock Curran Associates, Inc.

\bibitem[\protect\citeauthoryear{Levine \bgroup et al\mbox.\egroup
  }{2016}]{levine2016end}
Levine, S.; Finn, C.; Darrell, T.; and Abbeel, P.
\newblock 2016.
\newblock End-to-end training of deep visuomotor policies.
\newblock {\em The Journal of Machine Learning Research} 17(1):1334--1373.

\bibitem[\protect\citeauthoryear{Lewis \bgroup et al\mbox.\egroup
  }{2017}]{lewis-etal-2017-deal}
Lewis, M.; Yarats, D.; Dauphin, Y.; Parikh, D.; and Batra, D.
\newblock 2017.
\newblock {Deal or No Deal? End-to-End Learning of Negotiation Dialogues}.
\newblock In {\em Proceedings of the 2017 Conference on Empirical Methods in
  Natural Language Processing},  pp. 2443--2453.
\newblock Copenhagen, Denmark: Association for Computational Linguistics.

\bibitem[\protect\citeauthoryear{Li \bgroup et al\mbox.\egroup
  }{2016a}]{li2016deep}
Li, J.; Monroe, W.; Ritter, A.; Galley, M.; Gao, J.; and Jurafsky, D.
\newblock 2016a.
\newblock Deep reinforcement learning for dialogue generation.
\newblock {\em ArXiv:1606.01541}.

\bibitem[\protect\citeauthoryear{Li \bgroup et al\mbox.\egroup
  }{2016b}]{li2016user}
Li, X.; Lipton, Z.~C.; Dhingra, B.; Li, L.; Gao, J.; and Chen, Y.-N.
\newblock 2016b.
\newblock A user simulator for task-completion dialogues.
\newblock {\em ArXiv:1612.05688}.

\bibitem[\protect\citeauthoryear{Li \bgroup et al\mbox.\egroup
  }{2017a}]{li2017dialogue}
Li, J.; Miller, A.~H.; Chopra, S.; Ranzato, M.; and Weston, J.
\newblock 2017a.
\newblock Dialogue learning with human-in-the-loop.
\newblock In {\em Proceedings of the 5th International Conference on Learning
  Representations}.
\newblock Toulon, France: OpenReview.net.

\bibitem[\protect\citeauthoryear{Li \bgroup et al\mbox.\egroup
  }{2017b}]{li2017learning_to_learn}
Li, J.; Miller, A.~H.; Chopra, S.; Ranzato, M.; and Weston, J.
\newblock 2017b.
\newblock Learning through dialogue interactions by asking questions.
\newblock In {\em Proceedings of the 5th International Conference on Learning
  Representations}.
\newblock Toulon, France: OpenReview.net.

\bibitem[\protect\citeauthoryear{Li \bgroup et al\mbox.\egroup
  }{2017c}]{li2017end}
Li, X.; Chen, Y.-N.; Li, L.; Gao, J.; and Celikyilmaz, A.
\newblock 2017c.
\newblock End-to-end task-completion neural dialogue systems.
\newblock In {\em Proceedings of the The 8th International Joint Conference on
  Natural Language Processing},  pp. 733--743.
\newblock Taipei, Taiwan: AFNLP.

\bibitem[\protect\citeauthoryear{Li, Weston, and
  Roller}{2019}]{Li2019ACUTEEVALID}
Li, M.; Weston, J.; and Roller, S.
\newblock 2019.
\newblock {ACUTE-EVAL: Improved Dialogue Evaluation with Optimized Questions
  and Multi-turn Comparisons}.
\newblock In {\em 3rd Workshop on Conversational AI, NeurIPS}.

\bibitem[\protect\citeauthoryear{Lindgren}{1968}]{lindgren1968purposive}
Lindgren, N.
\newblock 1968.
\newblock {Purposive systems: The edge of knowledge}.
\newblock {\em IEEE spectrum} 5(4):89--100.

\bibitem[\protect\citeauthoryear{Lipton \bgroup et al\mbox.\egroup
  }{2018}]{lipton2018bbq}
Lipton, Z.; Li, X.; Gao, J.; Li, L.; Ahmed, F.; and Deng, L.
\newblock 2018.
\newblock {BBQ-networks: Efficient exploration in deep reinforcement learning
  for task-oriented dialogue systems}.
\newblock In {\em Thirty-Second AAAI Conference on Artificial Intelligence},
  pp. 5237--5244.

\bibitem[\protect\citeauthoryear{Lison}{2013}]{lison2013model}
Lison, P.
\newblock 2013.
\newblock Model-based bayesian reinforcement learning for dialogue management.
\newblock {\em ArXiv:1304.1819}.

\bibitem[\protect\citeauthoryear{ListNote}{2020}]{listNote}
ListNote.
\newblock 2020.
\newblock {ListNote Speech-to-Text Notes}.
\newblock {https://zapier.com/blog/best-text-dictation-software/#listnote}.

\bibitem[\protect\citeauthoryear{Litman \bgroup et al\mbox.\egroup
  }{2000}]{litman2000njfun}
Litman, D.; Singh, S.; Kearns, M.; and Walker, M.
\newblock 2000.
\newblock {NJFun: a reinforcement learning spoken dialogue system}.
\newblock In {\em ANLP-NAACL 2000 Workshop: Conversational Systems},  pp.
  17--20.

\bibitem[\protect\citeauthoryear{Littman and
  Sutton}{2001}]{littman2002predictive}
Littman, M.~L., and Sutton, R.~S.
\newblock 2001.
\newblock Predictive representations of state.
\newblock In {\em Proceedings of the 14th Conference on Advances in Neural
  Information Processing Systems},  pp. 1555--1561.
\newblock MIT Press.

\bibitem[\protect\citeauthoryear{Liu and Lane}{2017a}]{liu2017iterative}
Liu, B., and Lane, I.
\newblock 2017a.
\newblock Iterative policy learning in end-to-end trainable task-oriented
  neural dialog models.
\newblock In {\em Automatic Speech Recognition and Understanding Workshop,
  IEEE},  pp. 482--489.
\newblock IEEE.

\bibitem[\protect\citeauthoryear{Liu and Lane}{2017b}]{liu2017multi_domain}
Liu, B., and Lane, I.
\newblock 2017b.
\newblock Multi-domain adversarial learning for slot filling in spoken language
  understanding.
\newblock In {\em 1st Workshop on Conversational AI, NIPS}.

\bibitem[\protect\citeauthoryear{Liu \bgroup et al\mbox.\egroup
  }{2017}]{liu2017end}
Liu, B.; T{\"{u}}r, G.; Hakkani-T{\"{u}}r, D.; Shah, P.; and Heck, L.
\newblock 2017.
\newblock End-to-end optimization of task-oriented dialogue model with deep
  reinforcement learning.
\newblock {\em ArXiv:1711.10712}.

\bibitem[\protect\citeauthoryear{Liu \bgroup et al\mbox.\egroup
  }{2018}]{liu2018dialogue}
Liu, B.; T{\"{u}}r, G.; Hakkani-T{\"{u}}r, D.; Shah, P.; and Heck, L.
\newblock 2018.
\newblock Dialogue learning with human teaching and feedback in end-to-end
  trainable task-oriented dialogue systems.
\newblock In {\em Proceedings of NAACL-HLT},  pp. 2060--2069.
\newblock New Orleans, Louisiana: Association for Computational Linguistics.

\bibitem[\protect\citeauthoryear{Liu}{2018}]{bing2018_task_oriented}
Liu, B.
\newblock 2018.
\newblock {\em {Learning Task-Oriented Dialog with Neural Network Methods}}.
\newblock Ph.D. Dissertation, Carnegie Mellon University, Department of
  Electrical and Computer Engineering.

\bibitem[\protect\citeauthoryear{Loftin \bgroup et al\mbox.\egroup
  }{2014}]{loftin2014strategy}
Loftin, R.~T.; MacGlashan, J.; Peng, B.; Taylor, M.~E.; Littman, M.~L.; Huang,
  J.; and Roberts, D.~L.
\newblock 2014.
\newblock A strategy-aware technique for learning behaviors from discrete human
  feedback.
\newblock In {\em Twenty-Eighth AAAI Conference on Artificial Intelligence},
  pp. 937--943.

\bibitem[\protect\citeauthoryear{Long}{1981}]{long_1982_interaction}
Long, M.~H.
\newblock 1981.
\newblock Input, interaction and second language acquisition.
\newblock {\em Annals of the New York Academy of Sciences} 379(1):259--278.

\bibitem[\protect\citeauthoryear{Lu and Smith}{2007}]{lu_2007_e_commerce_asst}
Lu, Y., and Smith, S.
\newblock 2007.
\newblock {Augmented Reality E-Commerce Assistant System: Trying While
  Shopping}.
\newblock In Jacko, J.~A., ed., {\em Human-Computer Interaction. Interaction
  Platforms and Techniques},  pp. 643--652.
\newblock Berlin, Heidelberg: Springer Berlin Heidelberg.

\bibitem[\protect\citeauthoryear{Lucas, Miko, and
  Bennington}{2004}]{lucas2004method}
Lucas, M.; Miko, S.; and Bennington, S.~A.
\newblock 2004.
\newblock {\em Method and apparatus for voice dictation and document
  production}.
\newblock US Patent 6,834,264. Google Patents.

\bibitem[\protect\citeauthoryear{Madotto \bgroup et al\mbox.\egroup
  }{2019}]{madotto2020attention}
Madotto, A.; Lin, Z.; Wu, C.-S.; Shin, J.; and Fung, P.
\newblock 2019.
\newblock {Attention over Parameters for Dialogue Systems}.
\newblock In {\em 3rd Workshop on Conversational AI, NeurIPS}.

\bibitem[\protect\citeauthoryear{Maheswaran \bgroup et al\mbox.\egroup
  }{2003}]{maheswaran2003adjustable}
Maheswaran, R.~T.; Tambe, M.; Varakantham, P.; and Myers, K.
\newblock 2003.
\newblock Adjustable autonomy challenges in personal assistant agents: A
  position paper.
\newblock In {\em International Workshop on Computational Autonomy, AAMAS},
  pp. 187--194.
\newblock Springer.

\bibitem[\protect\citeauthoryear{Manuvinakurike \bgroup et al\mbox.\egroup
  }{2018}]{manuvinakurike2018conversational}
Manuvinakurike, R.; Bui, T.; Chang, W.; and Georgila, K.
\newblock 2018.
\newblock {Conversational image editing: Incremental intent identification in a
  new dialogue task}.
\newblock In {\em Proceedings of the 19th Annual SIGdial Meeting on Discourse
  and Dialogue},  pp. 284--295.

\bibitem[\protect\citeauthoryear{Mathewson and
  Pilarski}{2016}]{mathewson2016simultaneous}
Mathewson, K.~W., and Pilarski, P.~M.
\newblock 2016.
\newblock Simultaneous control and human feedback in the training of a robotic
  agent with actor-critic reinforcement learning.
\newblock In {\em Workshop on Interactive Machine Learning, IJCAI}.

\bibitem[\protect\citeauthoryear{McDermott}{1982}]{mcdermott1982xsel}
McDermott, J.
\newblock 1982.
\newblock {XSEL: A computer salesperson's assistant}.
\newblock {\em Machine intelligence} 10(1):235--337.

\bibitem[\protect\citeauthoryear{Mendez \bgroup et al\mbox.\egroup
  }{2019}]{mendez2019reinforcement}
Mendez, J.~A.; Geramifard, A.; Ghavamzadeh, M.; and Liu, B.
\newblock 2019.
\newblock {Reinforcement Learning of Multi-Domain Dialog Policies Via Action
  Embeddings}.
\newblock In {\em 3rd Workshop on Conversational AI, NeurIPS}.

\bibitem[\protect\citeauthoryear{{Microsoft}}{2020}]{microsoft}
{Microsoft}.
\newblock 2020.
\newblock {\em {Windows Speech Recognition commands}}.
\newblock
  {https://support.microsoft.com/en-ca/help/12427/windows-speech-recognition-commands}.
  Accessed February 23, 2020.

\bibitem[\protect\citeauthoryear{Mnih \bgroup et al\mbox.\egroup
  }{2013}]{mnih2013playing}
Mnih, V.; Kavukcuoglu, K.; Silver, D.; Graves, A.; Antonoglou, I.; Wierstra,
  D.; and Riedmiller, M.
\newblock 2013.
\newblock {Playing Atari with Deep Reinforcement Learning}.
\newblock In {\em Deep Learning Workshop, NIPS}.

\bibitem[\protect\citeauthoryear{Moore and Paris}{1989}]{moore1989planning}
Moore, J.~D., and Paris, C.~L.
\newblock 1989.
\newblock Planning text for advisory dialogues.
\newblock In {\em Proceedings of the 27th Annual Meeting on Association for
  Computational Linguistics},  pp. 203--211.
\newblock Association for Computational Linguistics.

\bibitem[\protect\citeauthoryear{Moore}{2015}]{moore2019}
Moore, A.
\newblock 2015.
\newblock Artificial {I}ntelligence: 10 {T}hings {T}o {K}now.

\bibitem[\protect\citeauthoryear{Mordatch and
  Abbeel}{2018}]{mordatch2018emergence}
Mordatch, I., and Abbeel, P.
\newblock 2018.
\newblock Emergence of grounded compositional language in multi-agent
  populations.
\newblock In {\em Thirty-Second AAAI Conference on Artificial Intelligence}.
\newblock AAAI.

\bibitem[\protect\citeauthoryear{Ng \bgroup et al\mbox.\egroup
  }{2004}]{ng_2003_helicopter}
Ng, A.~Y.; Kim, H.~J.; Jordan, M.~I.; and Sastry, S.
\newblock 2004.
\newblock Autonomous helicopter flight via reinforcement learning.
\newblock In Thrun, S.; Saul, L.~K.; and Sch\"{o}lkopf, B., eds., {\em
  Proceedings of the 16th Conference on Advances in Neural Information
  Processing Systems}. MIT Press.
\newblock  pp. 799--806.

\bibitem[\protect\citeauthoryear{Ng \bgroup et al\mbox.\egroup
  }{2006}]{ng2006autonomous}
Ng, A.~Y.; Coates, A.; Diel, M.; Ganapathi, V.; Schulte, J.; Tse, B.; Berger,
  E.; and Liang, E.
\newblock 2006.
\newblock Autonomous inverted helicopter flight via reinforcement learning.
\newblock In {\em Experimental robotics IX}. Springer.
\newblock  pp. 363--372.

\bibitem[\protect\citeauthoryear{Nonaka \bgroup et al\mbox.\egroup
  }{2012}]{nonaka2012towards}
Nonaka, Y.; Sakai, Y.; Yasuda, K.; and Nakano, Y.
\newblock 2012.
\newblock Towards assessing the communication responsiveness of people with
  dementia.
\newblock In {\em International Conference on Intelligent Virtual Agents},  pp.
  496--498.
\newblock Springer.

\bibitem[\protect\citeauthoryear{Nortmann \bgroup et al\mbox.\egroup
  }{2015}]{nortmann2015primary}
Nortmann, N.; Rekauzke, S.; Onat, S.; K{\"o}nig, P.; and Jancke, D.
\newblock 2015.
\newblock Primary visual cortex represents the difference between past and
  present.
\newblock {\em Cerebral Cortex} 25(6):1427--1440.

\bibitem[\protect\citeauthoryear{{Nuance Communications, Inc.}}{2020}]{nuance}
{Nuance Communications, Inc.}
\newblock 2020.
\newblock {Nuance Winscribe Dictation}.

\bibitem[\protect\citeauthoryear{Paolacci, Chandler, and
  Ipeirotis}{2010}]{paolacci2010running}
Paolacci, G.; Chandler, J.; and Ipeirotis, P.~G.
\newblock 2010.
\newblock {Running Experiments on Amazon Mechanical Turk}.
\newblock {\em Judgment and Decision making} 5(5):411--419.

\bibitem[\protect\citeauthoryear{Papangelis \bgroup et al\mbox.\egroup
  }{2020}]{papangelis2020plato}
Papangelis, A.; Namazifar, M.; Khatri, C.; Wang, Y.-C.; Molino, P.; and
  T{\"{u}}r, G.
\newblock 2020.
\newblock {Plato Dialogue System: A Flexible Conversational AI Research
  Platform}.
\newblock {\em ArXiv:2001.06463}.

\bibitem[\protect\citeauthoryear{Parr \bgroup et al\mbox.\egroup
  }{2008}]{parr2008analysis}
Parr, R.; Li, L.; Taylor, G.; Painter-Wakefield, C.; and Littman, M.~L.
\newblock 2008.
\newblock An analysis of linear models, linear value-function approximation,
  and feature selection for reinforcement learning.
\newblock In {\em Proceedings of the 25th international conference on Machine
  learning},  pp. 752--759.

\bibitem[\protect\citeauthoryear{Peng \bgroup et al\mbox.\egroup
  }{2017}]{peng2017composite}
Peng, B.; Li, X.; Li, L.; Gao, J.; Celikyilmaz, A.; Lee, S.; and Wong, K.-F.
\newblock 2017.
\newblock Composite task-completion dialogue policy learning via hierarchical
  deep reinforcement learning.
\newblock In {\em Proceedings of the Conference on Empirical Methods in Natural
  Language Processing},  pp. 2231--2240.
\newblock Copenhagen, Denmark: Association for Computational Linguistics.

\bibitem[\protect\citeauthoryear{Peng \bgroup et al\mbox.\egroup
  }{2018}]{Peng_2018deepdynaQ}
Peng, B.; Li, X.; Gao, J.; Liu, J.; and Wong, K.-F.
\newblock 2018.
\newblock {Deep Dyna-Q: Integrating Planning for Task-Completion Dialogue
  Policy Learning}.
\newblock In {\em Proceedings of the 56th Annual Meeting of the Association for
  Computational Linguistics (Volume 1: Long Papers)}.
\newblock Association for Computational Linguistics.

\bibitem[\protect\citeauthoryear{Pica, Doughty, and
  Young}{1986}]{pica1986making}
Pica, T.; Doughty, C.~J.; and Young, R.
\newblock 1986.
\newblock {Making input comprehensible: Do interactional modifications help?}
\newblock {\em ITL-International Journal of Applied Linguistics} 72(1):1--25.

\bibitem[\protect\citeauthoryear{Pica}{1987}]{pica1987second}
Pica, T.
\newblock 1987.
\newblock Second-language acquisition, social interaction, and the classroom.
\newblock {\em Applied linguistics} 8(1):3--21.

\bibitem[\protect\citeauthoryear{Pilarski and
  Sutton}{2012}]{pilarski2012between}
Pilarski, P.~M., and Sutton, R.~S.
\newblock 2012.
\newblock Between instruction and reward: human-prompted switching.
\newblock Technical Report FS-12-07, AAAI 2012 Fall Symposium on Robots
  Learning Interactively from Human Teachers (RLIHT), Arlington, VA.

\bibitem[\protect\citeauthoryear{Pilarski \bgroup et al\mbox.\egroup
  }{2011}]{pilarski2011online}
Pilarski, P.~M.; Dawson, M.~R.; Degris, T.; Fahimi, F.; Carey, J.~P.; and
  Sutton, R.~S.
\newblock 2011.
\newblock Online human training of a myoelectric prosthesis controller via
  actor-critic reinforcement learning.
\newblock In {\em Proceedings of the IEEE International Conference on
  Rehabilitation Robotics},  pp. 134--140.
\newblock Zurich, Switzerland: IEEE.

\bibitem[\protect\citeauthoryear{Pilarski \bgroup et al\mbox.\egroup
  }{2017}]{pilarski2017communicative}
Pilarski, P.~M.; Sutton, R.~S.; Mathewson, K.~W.; Sherstan, C.; Parker, A.~S.;
  and Edwards, A.~L.
\newblock 2017.
\newblock {Communicative Capital for Prosthetic Agents}.
\newblock {\em ArXiv:1711.03676}.

\bibitem[\protect\citeauthoryear{Pilarski, Sutton, and
  Mathewson}{2015}]{pilarski2015prosthetic}
Pilarski, P.~M.; Sutton, R.~S.; and Mathewson, K.~W.
\newblock 2015.
\newblock Prosthetic devices as goal-seeking agents.
\newblock In {\em Second Workshop on Present and Future of Non-Invasive
  Peripheral-Nervous-System Machine Interfaces: Progress in Restoring the Human
  Functions, PNS-MI}.

\bibitem[\protect\citeauthoryear{Pineau \bgroup et al\mbox.\egroup
  }{2003}]{pineau2003towards}
Pineau, J.; Montemerlo, M.; Pollack, M.; Roy, N.; and Thrun, S.
\newblock 2003.
\newblock Towards robotic assistants in nursing homes: Challenges and results.
\newblock {\em Robotics and autonomous systems} 42(3-4):271--281.

\bibitem[\protect\citeauthoryear{Pollack \bgroup et al\mbox.\egroup
  }{2002}]{pollack2002pearl}
Pollack, M.~E.; Brown, L.; Colbry, D.; Orosz, C.; Peintner, B.; Ramakrishnan,
  S.; Engberg, S.; Matthews, J.~T.; Dunbar-Jacob, J.; McCarthy, C.~E.; et~al.
\newblock 2002.
\newblock {Pearl: A mobile robotic assistant for the elderly}.
\newblock In {\em Workshop on automation as eldercare, AAAI},  pp. 85--91.

\bibitem[\protect\citeauthoryear{Pollack, Hirschberg, and
  Webber}{1982}]{pollack1982user}
Pollack, M.~E.; Hirschberg, J.; and Webber, B.
\newblock 1982.
\newblock User participation in the reasoning processes of expert systems.
\newblock In {\em Proceedings First National Conference on Artificial
  Intelligence (AAAI-82)},  pp. 358--361.
\newblock University of Pennsylvania.

\bibitem[\protect\citeauthoryear{Poole and
  Mackworth}{2010}]{poole2010artificial}
Poole, D.~L., and Mackworth, A.~K.
\newblock 2010.
\newblock {\em Artificial Intelligence: foundations of computational agents}.
\newblock Cambridge University Press.

\bibitem[\protect\citeauthoryear{Power}{1974}]{power1974computer}
Power, R.
\newblock 1974.
\newblock {\em A computer model of conversation}.
\newblock Ph.D. Dissertation, The University of Edinburg.

\bibitem[\protect\citeauthoryear{Quarteroni and
  Manandhar}{2009}]{quarteroni2009designing}
Quarteroni, S., and Manandhar, S.
\newblock 2009.
\newblock Designing an interactive open-domain question answering system.
\newblock {\em Natural Language Engineering} 15(1):73--95.

\bibitem[\protect\citeauthoryear{Radford \bgroup et al\mbox.\egroup
  }{2019}]{radford2019language}
Radford, A.; Wu, J.; Child, R.; Luan, D.; Amodei, D.; and Sutskever, I.
\newblock 2019.
\newblock Language models are unsupervised multitask learners.
\newblock {\em OpenAI Blog}.
\newblock {https://openai.com/blog/better-language-models}. [Accessed July 23,
  2020].

\bibitem[\protect\citeauthoryear{Ranzato \bgroup et al\mbox.\egroup
  }{2015}]{ranzato2015sequence}
Ranzato, M.; Chopra, S.; Auli, M.; and Zaremba, W.
\newblock 2015.
\newblock Sequence level training with recurrent neural networks.
\newblock {\em ArXiv:1511.06732}.

\bibitem[\protect\citeauthoryear{Rao}{2011}]{rao2011predictive}
Rao, A.~P.
\newblock 2011.
\newblock {\em Predictive speech-to-text input}.
\newblock US Patent 7,904,298. Google Patents.

\bibitem[\protect\citeauthoryear{Rastogi, Hakkani-T{\"u}r, and
  Heck}{2017}]{rastogi2017scalable}
Rastogi, A.; Hakkani-T{\"u}r, D.; and Heck, L.
\newblock 2017.
\newblock Scalable multi-domain dialogue state tracking.
\newblock In {\em IEEE Automatic Speech Recognition and Understanding Workshop
  (ASRU)},  pp. 561--568.
\newblock IEEE.

\bibitem[\protect\citeauthoryear{Rumelhart \bgroup et al\mbox.\egroup
  }{1986}]{rumelhart1986sequential}
Rumelhart, D.~E.; Smolensky, P.; McClelland, J.~L.; and Hinton, G.
\newblock 1986.
\newblock {Sequential thought processes in PDP models}.
\newblock {\em Parallel Distributed Processing: Explorations in the
  Microstructures of Cognition} 2:pp. 7--57.
\newblock MIT Press.

\bibitem[\protect\citeauthoryear{Saleh \bgroup et al\mbox.\egroup
  }{2019}]{saleh2019hierarchical}
Saleh, A.; Jaques, N.; Ghandeharioun, A.; Shen, J.~H.; and Picard, R.
\newblock 2019.
\newblock Hierarchical reinforcement learning for open-domain dialog.
\newblock In {\em 3rd Workshop on Conversational AI, NeurIPS}.

\bibitem[\protect\citeauthoryear{Salichs \bgroup et al\mbox.\egroup
  }{2019}]{salichs2019preface}
Salichs, M.~A.; Ge, S.~S.; Barakova, E.; Cabibihan, J.-J.; Wagner, A.~R.;
  Gonzalez, A.~C.; and He, H., eds.
\newblock 2019.
\newblock {\em {Preface--Social Robotics: 11th International Conference,
  ICSR}}.
\newblock Springer.

\bibitem[\protect\citeauthoryear{Schatzmann \bgroup et al\mbox.\egroup
  }{2007}]{schatzmann2007agenda}
Schatzmann, J.; Thomson, B.; Weilhammer, K.; Ye, H.; and Young, S.
\newblock 2007.
\newblock Agenda-based user simulation for bootstrapping a {POMDP} dialogue
  system.
\newblock In {\em Human Language Technologies 2007: The Conference of the North
  American Chapter of the Association for Computational Linguistics; Companion
  Volume, Short Papers},  pp. 149--152.
\newblock Association for Computational Linguistics.

\bibitem[\protect\citeauthoryear{Schrittwieser \bgroup et al\mbox.\egroup
  }{2019}]{schrittwieser2019mastering}
Schrittwieser, J.; Antonoglou, I.; Hubert, T.; Simonyan, K.; Sifre, L.;
  Schmitt, S.; Guez, A.; Lockhart, E.; Hassabis, D.; Graepel, T.; Lillicrap,
  T.; and Silver, D.
\newblock 2019.
\newblock {Mastering Atari, Go, chess and shogi by planning with a learned
  model}.
\newblock In {\em Proceedings of the Thirty-third Conference on Neural
  Information Processing Systems}.
\newblock Vancouver, Canada: Curran Associates, Inc.

\bibitem[\protect\citeauthoryear{Selfridge}{1993}]{selfridge1993gardens}
Selfridge, O.~G.
\newblock 1993.
\newblock {The Gardens of Learning: A Vision for AI}.
\newblock {\em AI Magazine} 14(2):36--48.

\bibitem[\protect\citeauthoryear{Serban \bgroup et al\mbox.\egroup
  }{2017a}]{serban2017deep}
Serban, I.~V.; Sankar, C.; Germain, M.; Zhang, S.; Lin, Z.; Subramanian, S.;
  Kim, T.; Pieper, M.; Chandar, S.; Ke, N.~R.; et~al.
\newblock 2017a.
\newblock A deep reinforcement learning chatbot.
\newblock {\em ArXiv:1709.02349}.

\bibitem[\protect\citeauthoryear{Serban \bgroup et al\mbox.\egroup
  }{2017b}]{serban2017hierarchical}
Serban, I.~V.; Sordoni, A.; Lowe, R.; Charlin, L.; Pineau, J.; Courville, A.;
  and Bengio, Y.
\newblock 2017b.
\newblock A hierarchical latent variable encoder-decoder model for generating
  dialogues.
\newblock In {\em Proceedings of the Thirty-First AAAI Conference on Artificial
  Intelligence},  pp. 3295--3301.
\newblock AAAI.

\bibitem[\protect\citeauthoryear{Shah \bgroup et al\mbox.\egroup
  }{2018}]{shah2018building_self_play}
Shah, P.; Hakkani-T{\"u}r, D.; T{\"u}r, G.; Rastogi, A.; Bapna, A.; Nayak, N.;
  and Heck, L.
\newblock 2018.
\newblock Building a conversational agent overnight with dialogue self-play.
\newblock {\em ArXiv:1801.04871}.

\bibitem[\protect\citeauthoryear{Shah, Hakkani-T{\"{u}}r, and
  Heck}{2016}]{shah2016interactive}
Shah, P.; Hakkani-T{\"{u}}r, D.; and Heck, L.
\newblock 2016.
\newblock Interactive reinforcement learning for task-oriented dialogue
  management.
\newblock In {\em Workshop on Deep Learning for Action and Interaction, NIPS}.

\bibitem[\protect\citeauthoryear{Shen \bgroup et al\mbox.\egroup
  }{2017}]{shen2017reasonet}
Shen, Y.; Huang, P.-S.; Gao, J.; and Chen, W.
\newblock 2017.
\newblock {ReasoNet: Learning to Stop Reading in Machine Comprehension}.
\newblock In {\em Proceedings of the 23rd ACM SIGKDD International Conference
  on Knowledge Discovery and Data Mining},  pp. 1047--1055.

\bibitem[\protect\citeauthoryear{Shi \bgroup et al\mbox.\egroup
  }{2018}]{Shi_2018}
Shi, Z.; Chen, X.; Qiu, X.; and Huang, X.
\newblock 2018.
\newblock {Toward Diverse Text Generation with Inverse Reinforcement Learning}.
\newblock {\em Proceedings of the Twenty-Seventh International Joint Conference
  on Artificial Intelligence}.

\bibitem[\protect\citeauthoryear{Shin \bgroup et al\mbox.\egroup
  }{2019}]{shin2019happybot}
Shin, J.; Xu, P.; Madotto, A.; and Fung, P.
\newblock 2019.
\newblock {Happybot: Generating empathetic dialogue responses by improving user
  experience look-ahead}.
\newblock {\em ArXiv:1906.08487}.

\bibitem[\protect\citeauthoryear{Shu \bgroup et al\mbox.\egroup
  }{2018}]{shu2018incorporating}
Shu, L.; Molino, P.; Namazifar, M.; Liu, B.; Xu, H.; Zheng, H.; and T{\"{u}}r,
  G.
\newblock 2018.
\newblock Incorporating the structure of the belief state in end-to-end
  task-oriented dialogue systems.
\newblock In {\em 2nd Workshop on Conversational AI, NIPS}, volume~32.

\bibitem[\protect\citeauthoryear{Silver \bgroup et al\mbox.\egroup
  }{2017a}]{silver2017mastering}
Silver, D.; Schrittwieser, J.; Simonyan, K.; Antonoglou, I.; Huang, A.; Guez,
  A.; Hubert, T.; Baker, L.; Lai, M.; Bolton, A.; et~al.
\newblock 2017a.
\newblock {Mastering the game of Go without human knowledge}.
\newblock {\em Nature} 550(7676):354--359.

\bibitem[\protect\citeauthoryear{Silver \bgroup et al\mbox.\egroup
  }{2017b}]{silver2017predictron}
Silver, D.; van Hasselt, H.; Hessel, M.; Schaul, T.; Guez, A.; Harley, T.;
  Dulac-Arnold, G.; Reichert, D.; Rabinowitz, N.; Barreto, A.; et~al.
\newblock 2017b.
\newblock {The Predictron: End-to-end learning and planning}.
\newblock In {\em Proceedings of the 34th International Conference on Machine
  Learning-Volume 70},  pp. 3191--3199.
\newblock JMLR. org.

\bibitem[\protect\citeauthoryear{Silver \bgroup et al\mbox.\egroup
  }{2018}]{silver2018general}
Silver, D.; Hubert, T.; Schrittwieser, J.; Antonoglou, I.; Lai, M.; Guez, A.;
  Lanctot, M.; Sifre, L.; Kumaran, D.; Graepel, T.; Lillicrap, T.; Simonyan,
  K.; and Hassabis, D.
\newblock 2018.
\newblock {A general reinforcement learning algorithm that masters chess,
  shogi, and Go through self-play}.
\newblock {\em Science} 362(6419):1140--1144.

\bibitem[\protect\citeauthoryear{Simmons and
  Slocum}{1972}]{simmons1972generating}
Simmons, R., and Slocum, J.
\newblock 1972.
\newblock {Generating English discourse from semantic networks}.
\newblock {\em Communications of the ACM} 15(10):891--905.

\bibitem[\protect\citeauthoryear{Singh \bgroup et al\mbox.\egroup
  }{2000}]{singh2000reinforcement}
Singh, S.~P.; Kearns, M.~J.; Litman, D.~J.; and Walker, M.~A.
\newblock 2000.
\newblock Reinforcement learning for spoken dialogue systems.
\newblock In {\em Proceedings of the 13th Conference on Advances in Neural
  Information Processing Systems},  pp. 956--962.

\bibitem[\protect\citeauthoryear{Singh \bgroup et al\mbox.\egroup
  }{2002a}]{singh2002optimizingNJFun}
Singh, S.; Litman, D.; Kearns, M.; and Walker, M.
\newblock 2002a.
\newblock Optimizing dialogue management with reinforcement learning:
  {E}xperiments with the {NJF}un system.
\newblock {\em Journal of Artificial Intelligence Research} 16:105--133.

\bibitem[\protect\citeauthoryear{Singh \bgroup et al\mbox.\egroup
  }{2002b}]{singh2002optimizing}
Singh, S.; Litman, D.; Kearns, M.; and Walker, M.
\newblock 2002b.
\newblock Optimizing dialogue management with reinforcement learning:
  Experiments with the {NJF}un system.
\newblock {\em Artificial Intelligence} 16:pp. 105--133.

\bibitem[\protect\citeauthoryear{Singh}{1992}]{singh1992_h_dyna}
Singh, S.~P.
\newblock 1992.
\newblock Reinforcement learning with a hierarchy of abstract models.
\newblock In {\em Proceedings of the National Conference on Artificial
  Intelligence}, number~10,  p.202.
\newblock Citeseer.

\bibitem[\protect\citeauthoryear{Skantze}{2016}]{skantze2016real}
Skantze, G.
\newblock 2016.
\newblock Real-time coordination in human-robot interaction using face and
  voice.
\newblock {\em AI Magazine} 37(4):19--31.

\bibitem[\protect\citeauthoryear{Smith and Hipp}{1994}]{smith1994spoken}
Smith, R.~W., and Hipp, D.~R.
\newblock 1994.
\newblock {\em Spoken natural language dialog systems: {A} practical approach}.
\newblock Oxford University Press.

\bibitem[\protect\citeauthoryear{Smith \bgroup et al\mbox.\egroup
  }{2020}]{smith2020can_openDomain}
Smith, E.~M.; Williamson, M.; Shuster, K.; Weston, J.; and Boureau, Y.-L.
\newblock 2020.
\newblock {Can You Put it All Together: Evaluating Conversational Agents'
  Ability to Blend Skills}.
\newblock {\em ArXiv:2004.08449}.

\bibitem[\protect\citeauthoryear{Stent, Prasad, and
  Walker}{2004}]{stent_2004_planning}
Stent, A.; Prasad, R.; and Walker, M.
\newblock 2004.
\newblock Trainable sentence planning for complex information presentation in
  spoken dialog systems.
\newblock In {\em Proceedings of the 42nd Annual Meeting on Association for
  Computational Linguistics}, ACL ’04,  pp. 79--–87.
\newblock Barcelona, Spain: Association for Computational Linguistics.

\bibitem[\protect\citeauthoryear{Su \bgroup et al\mbox.\egroup
  }{2016}]{su2016continuously}
Su, P.-H.; Ga\v{s}i\'{c}, M.; Mrk\v{s}ic, N.; Rojas-Barahona, L.; Ultes, S.;
  Vandyke, D.; Wen, T.-H.; and Young, S.
\newblock 2016.
\newblock Continuously learning neural dialogue management.
\newblock {\em ArXiv:1606.02689}.

\bibitem[\protect\citeauthoryear{Su \bgroup et al\mbox.\egroup
  }{2017}]{su2017sample}
Su, P.-H.; Budzianowski, P.; Ultes, S.; Ga\v{s}i\'{c}, M.; and Young, S.
\newblock 2017.
\newblock Sample-efficient actor-critic reinforcement learning with supervised
  data for dialogue management.
\newblock In {\em Proceedings of the SIGDIAL 2017 Conference},  pp. 147--157.

\bibitem[\protect\citeauthoryear{Su \bgroup et al\mbox.\egroup
  }{2018}]{su-etal-2018-discriminativeDynaQ}
Su, S.-Y.; Li, X.; Gao, J.; Liu, J.; and Chen, Y.-N.
\newblock 2018.
\newblock {Discriminative Deep {Dyna-Q}: Robust Planning for Dialogue Policy
  Learning}.
\newblock In {\em Proceedings of the 2018 Conference on Empirical Methods in
  Natural Language Processing},  pp. 3813--3823.
\newblock Brussels, Belgium: Association for Computational Linguistics.

\bibitem[\protect\citeauthoryear{Sukhbaatar, Szlam, and
  Fergus}{2016}]{sukhbaatar2016learning}
Sukhbaatar, S.; Szlam, A.; and Fergus, R.
\newblock 2016.
\newblock Learning multiagent communication with backpropagation.
\newblock In {\em Proceedings of the 30th Conference on Advances in Neural
  Information Processing Systems},  pp. 2244--2252.

\bibitem[\protect\citeauthoryear{Sun, Chen, and
  Rudnicky}{2016}]{sun2016intelligent}
Sun, M.; Chen, Y.-N.; and Rudnicky, A.~I.
\newblock 2016.
\newblock An intelligent assistant for high-level task understanding.
\newblock In {\em Proceedings of the 21st International Conference on
  Intelligent User Interfaces},  pp. 169--174.
\newblock Sonoma, USA: ACM.

\bibitem[\protect\citeauthoryear{Sutskever, Vinyals, and
  Le}{2014}]{sutskever2014sequence}
Sutskever, I.; Vinyals, O.; and Le, Q.~V.
\newblock 2014.
\newblock Sequence to sequence learning with neural networks.
\newblock In {\em Proceedings of the 28th Conference on Advances in neural
  information processing systems},  pp. 3104--3112.

\bibitem[\protect\citeauthoryear{Sutton and Barto}{1981}]{sutton1981adaptive}
Sutton, R.~S., and Barto, A.~G.
\newblock 1981.
\newblock An adaptive network that constructs and uses and internal model of
  its world.
\newblock {\em Cognition and Brain Theory} 4(3):217--246.

\bibitem[\protect\citeauthoryear{Sutton and
  Barto}{2018}]{sutton2018reinforcement}
Sutton, R.~S., and Barto, A.~G.
\newblock 2018.
\newblock {\em Reinforcement learning: An introduction}.
\newblock MIT press.

\bibitem[\protect\citeauthoryear{Sutton and Pinette}{1985}]{sutton1985learning}
Sutton, R.~S., and Pinette, B.
\newblock 1985.
\newblock The learning of world models by connectionist networks.
\newblock In {\em Proceedings of the seventh annual conference of the cognitive
  science society},  pp. 54--64.

\bibitem[\protect\citeauthoryear{Sutton \bgroup et al\mbox.\egroup
  }{2008}]{sutton2008dyna}
Sutton, R.~S.; Szepesv{\'a}ri, C.; Geramifard, A.; and Bowling, M.~P.
\newblock 2008.
\newblock Dyna-style planning with linear function approximation and
  prioritized sweeping.
\newblock In {\em Proceedings of the 24th Conference on Uncertainty in
  Artificial Intelligence},  pp. 528--536.

\bibitem[\protect\citeauthoryear{Sutton, Singh, and
  Precup}{1999}]{sutton1998between}
Sutton, R.~S.; Singh, S.; and Precup, D.
\newblock 1999.
\newblock Between {MDP}s and semi-{MDP}s: Learning, planning, and representing
  knowledge at multiple temporal scales.
\newblock {\em Artificial Intelligence} 112:118--211.

\bibitem[\protect\citeauthoryear{Sutton}{1990}]{sutton1990integrated}
Sutton, R.~S.
\newblock 1990.
\newblock Integrated architectures for learning, planning, and reacting based
  on approximating dynamic programming.
\newblock In {\em Proceedings of the Seventh International Conference on
  Machine Learning},  pp. 216--224.
\newblock Morgan Kaufmann.

\bibitem[\protect\citeauthoryear{Sutton}{2019}]{sutton2019MBRL}
Sutton, R.~S.
\newblock 2019.
\newblock Toward a {N}ew {A}pproach to {M}odel-based {R}einforcement
  {L}earning.
\newblock Technical report, University of Alberta.

\bibitem[\protect\citeauthoryear{Sutton}{2020}]{sutton2020VectorTalkMBRL}
Sutton, R.~S.
\newblock 2020.
\newblock {Experience and Intelligence: Toward a Scalable AI-Agent
  Architecture}.
\newblock Vector Institute for Artificial Intelligence, Visitor Talk.

\bibitem[\protect\citeauthoryear{Takahashi}{2001}]{takahashi2001document}
Takahashi, F.
\newblock 2001.
\newblock {\em Document editing system and method}.
\newblock US Patent 6,202,073. Google Patents.

\bibitem[\protect\citeauthoryear{Tang \bgroup et al\mbox.\egroup
  }{2018}]{tang2018subgoal}
Tang, D.; Li, X.; Gao, J.; Wang, C.; Li, L.; and Jebara, T.
\newblock 2018.
\newblock Subgoal discovery for hierarchical dialogue policy learning.
\newblock {\em ArXiv:1804.07855}.

\bibitem[\protect\citeauthoryear{Thomaz, Hoffman, and
  Breazeal}{2005}]{thomaz2005real}
Thomaz, A.~L.; Hoffman, G.; and Breazeal, C.
\newblock 2005.
\newblock Real-time interactive reinforcement learning for robots.
\newblock In {\em Workshop on human comprehensible machine learning, AAAI}.

\bibitem[\protect\citeauthoryear{Thomaz, Hoffman, and
  Breazeal}{2006}]{thomaz2006reinforcement}
Thomaz, A.~L.; Hoffman, G.; and Breazeal, C.
\newblock 2006.
\newblock {Reinforcement Learning with Human Teachers: Understanding How People
  Want to Teach Robots}.
\newblock In {\em The 15th {IEEE} International Symposium on Robot and Human
  Interactive Communication, {RO-MAN} 2006},  pp. 352--357.
\newblock IEEE.

\bibitem[\protect\citeauthoryear{Thompson}{2006}]{thompson2006google}
Thompson, C.
\newblock 2006.
\newblock {Google's China Problem}.
\newblock {\em The Power of Information.}
\newblock School of Journalism, Stony Brook University.

\bibitem[\protect\citeauthoryear{Todorov, Erez, and
  Tassa}{2012}]{todorov2012mujoco}
Todorov, E.; Erez, T.; and Tassa, Y.
\newblock 2012.
\newblock Mujoco: A physics engine for model-based control.
\newblock In {\em IEEE/RSJ International Conference on Intelligent Robots and
  Systems},  pp. 5026--5033.
\newblock IEEE.

\bibitem[\protect\citeauthoryear{Tractica}{2016}]{trac}
Tractica.
\newblock 2016.
\newblock {\em The {V}irtual {D}igital {A}ssistant {M}arket {W}ill {R}each
  \$15.8 {B}illion {W}orldwide by 2021}.
\newblock A market intelligence firm.
  {https://www.tractica.com/newsroom/press-releases/the-virtual-digital-assistant-market-will-reach-15-8-billion-worldwide-by-2021/}
  Accessed [July 23, 2020].

\bibitem[\protect\citeauthoryear{T{\"{u}}r \bgroup et al\mbox.\egroup
  }{2010}]{tur2010calo}
T{\"{u}}r, G.; Stolcke, A.; Voss, L.; Peters, S.; Hakkani-T{\"u}r, D.; Dowding,
  J.; Favre, B.; Fern{\'a}ndez, R.; Frampton, M.; Frandsen, M.; et~al.
\newblock 2010.
\newblock {The CALO Meeting Assistant System}.
\newblock {\em IEEE Transactions on Audio, Speech, and Language Processing}
  18(6):1601--1611.

\bibitem[\protect\citeauthoryear{T{\"{u}}r, Hakkani-T{\"u}r, and
  Schapire}{2005}]{tur2005combining}
T{\"{u}}r, G.; Hakkani-T{\"u}r, D.; and Schapire, R.~E.
\newblock 2005.
\newblock Combining active and semi-supervised learning for spoken language
  understanding.
\newblock {\em Speech Communication} 45(2):171--186.

\bibitem[\protect\citeauthoryear{Veeriah, Pilarski, and
  Sutton}{2016}]{veeriah2016face}
Veeriah, V.; Pilarski, P.~M.; and Sutton, R.~S.
\newblock 2016.
\newblock Face valuing: Training user interfaces with facial expressions and
  reinforcement learning.
\newblock In {\em Workshop on Interactive Machine Learning, IJCAI}.

\bibitem[\protect\citeauthoryear{Wahlstr{\"o}m, Sch{\"o}n, and
  Deisenroth}{2015}]{wahlstrom2015pixels}
Wahlstr{\"o}m, N.; Sch{\"o}n, T.~B.; and Deisenroth, M.~P.
\newblock 2015.
\newblock {From pixels to torques: Policy learning with deep dynamical models}.
\newblock {\em ArXiv:1502.02251}.

\bibitem[\protect\citeauthoryear{Walker and
  Grosz}{1978}]{walker1978understanding}
Walker, D.~E., and Grosz, B.~J.
\newblock 1978.
\newblock {\em Understanding spoken language}.
\newblock Elsevier Science Inc.

\bibitem[\protect\citeauthoryear{Walker \bgroup et al\mbox.\egroup
  }{2007}]{walker2007individual}
Walker, M.~A.; Stent, A.; Mairesse, F.; and Prasad, R.
\newblock 2007.
\newblock Individual and domain adaptation in sentence planning for dialogue.
\newblock {\em Journal of Artificial Intelligence Research} 30:413--456.

\bibitem[\protect\citeauthoryear{Walker}{1998}]{walker1998text}
Walker, R.~C.
\newblock 1998.
\newblock {\em Text processor}.
\newblock US Patent 5,802,533. Google Patents.

\bibitem[\protect\citeauthoryear{Walker}{2000}]{walker2000application}
Walker, M.~A.
\newblock 2000.
\newblock An application of reinforcement learning to dialogue strategy
  selection in a spoken dialogue system for email.
\newblock {\em Journal of Artificial Intelligence Research} 12:pp. 387--416.

\bibitem[\protect\citeauthoryear{Wang \bgroup et al\mbox.\egroup
  }{2016}]{wang2015dueling}
Wang, Z.; Schaul, T.; Hessel, M.; Van~Hasselt, H.; Lanctot, M.; and De~Freitas,
  N.
\newblock 2016.
\newblock Dueling network architectures for deep reinforcement learning.
\newblock In {\em Proceedings of the 33 rd International Conference on Machine
  Learning}, volume~48.
\newblock New York, USA: JMLR: W&CP.

\bibitem[\protect\citeauthoryear{Wang \bgroup et al\mbox.\egroup
  }{2019}]{wang2019hscjn}
Wang, Y.; Si, P.; Lei, Z.; Xun, G.; and Yang, Y.
\newblock 2019.
\newblock {HSCJN: A Holistic Semantic Constraint Joint Network for Diverse
  Response Generation}.
\newblock In {\em 3rd Workshop on Conversational AI, NeurIPS}.

\bibitem[\protect\citeauthoryear{Waters}{1986}]{waters1986kbemacs}
Waters, R.~C.
\newblock 1986.
\newblock {KBE}macs: Where's the {AI}?
\newblock {\em AI Magazine} 7(1):47--47.

\bibitem[\protect\citeauthoryear{Watter \bgroup et al\mbox.\egroup
  }{2015}]{watter2015embed}
Watter, M.; Springenberg, J.; Boedecker, J.; and Riedmiller, M.
\newblock 2015.
\newblock {Embed to control: A locally linear latent dynamics model for control
  from raw images}.
\newblock In {\em Proceedings of the 28th International Conference on Neural
  Information Processing Systems},  pp. 2746--2754.
\newblock Cambridge,USA: MIT Press.

\bibitem[\protect\citeauthoryear{Weisz \bgroup et al\mbox.\egroup
  }{2018}]{weisz2018sample}
Weisz, G.; Budzianowski, P.; Su, P.-H.; and Ga{\v{s}}i{\'c}, M.
\newblock 2018.
\newblock Sample efficient deep reinforcement learning for dialogue systems
  with large action spaces.
\newblock {\em IEEE/ACM Transactions on Audio, Speech, and Language Processing}
  26(11):2083--2097.

\bibitem[\protect\citeauthoryear{Wen \bgroup et al\mbox.\egroup
  }{2017}]{Wen_2017Gasic}
Wen, T.-H.; Vandyke, D.; Mrk\v{s}ic, N.; Ga\v{s}i\'{c}, M.; Rojas~Barahona,
  L.~M.; Su, P.-H.; Ultes, S.; and Young, S.
\newblock 2017.
\newblock {A Network-based End-to-End Trainable Task-oriented Dialogue System}.
\newblock In {\em Proceedings of the 15th Conference of the European Chapter of
  the Association for Computational Linguistics: Volume 1, Long Papers},  pp.
  437--449.
\newblock Valencia, Spain: Association for Computational Linguistics.

\bibitem[\protect\citeauthoryear{Wiering, Salustowicz, and
  Schmidhuber}{2001}]{wiering2001model}
Wiering, M.; Salustowicz, R.; and Schmidhuber, J.
\newblock 2001.
\newblock Model-based reinforcement learning for evolving soccer strategies.
\newblock In {\em Computational intelligence in games},  pp. 99--132.
\newblock Springer.

\bibitem[\protect\citeauthoryear{Williams, Asadi, and
  Zweig}{2017}]{williams2017hybrid}
Williams, J.~D.; Asadi, K.; and Zweig, G.
\newblock 2017.
\newblock Hybrid code networks: practical and efficient end-to-end dialog
  control with supervised and reinforcement learning.
\newblock In {\em Proceedings of the 55th Annual Meeting of the Association for
  Computational Linguistics}.
\newblock Association for Computational Linguistics.

\bibitem[\protect\citeauthoryear{Winograd}{1971}]{winograd1971procedures}
Winograd, T.
\newblock 1971.
\newblock Procedures as a representation for data in a computer program for
  understanding natural language.
\newblock Technical report, MIT.

\bibitem[\protect\citeauthoryear{Winograd}{1973}]{winograd1973breaking}
Winograd, T.
\newblock 1973.
\newblock Breaking the complexity barrier again.
\newblock In {\em ACM SIGIR Forum}, volume~9,  pp. 13--30.
\newblock ACM.
\newblock Reprinted in David R. Barstow, Howard E. Shrobe, and Erik Sandewall
  (Eds.), {\it Interactive Programming Environments}, McGraw-Hill Book Co., New
  York, 1984.

\bibitem[\protect\citeauthoryear{Woodrow}{1946}]{WoodrowH.1946Tatl}
Woodrow, H.
\newblock 1946.
\newblock The ability to learn.
\newblock {\em Psychological Review} 53(3):147--158.

\bibitem[\protect\citeauthoryear{Woods}{1984}]{woods1984natural}
Woods, W.
\newblock 1984.
\newblock Natural language communication with machines: An ongoing goal.
\newblock {\em Artificial intelligence applications for business}  pp.
  195--209.

\bibitem[\protect\citeauthoryear{Wu \bgroup et al\mbox.\egroup
  }{2019}]{wu2019switch}
Wu, Y.; Li, X.; Liu, J.; Gao, J.; and Yang, Y.
\newblock 2019.
\newblock {Switch-based active deep Dyna-Q: Efficient adaptive planning for
  task-completion dialogue policy learning}.
\newblock In {\em Proceedings of the AAAI Conference on Artificial
  Intelligence}, volume~33,  pp. 7289--7296.

\bibitem[\protect\citeauthoryear{Xu, Wu, and Wu}{2018}]{xu2018towards}
Xu, C.; Wu, W.; and Wu, Y.
\newblock 2018.
\newblock Towards explainable and controllable open domain dialogue generation
  with dialogue acts.
\newblock {\em ArXiv:1807.07255}.

\bibitem[\protect\citeauthoryear{Yarats and
  Lewis}{2017}]{yarats2017hierarchical}
Yarats, D., and Lewis, M.
\newblock 2017.
\newblock {Hierarchical Text Generation and Planning for Strategic Dialogue}.
\newblock In {\em Proceedings of the 35th International Conference on Machine
  Learning}.
\newblock Stockholm, Sweden: PMRL 80.

\bibitem[\protect\citeauthoryear{Young \bgroup et al\mbox.\egroup
  }{2013}]{young2013pomdp}
Young, S.; Ga{\v{s}}i{\'c}, M.; Thomson, B.; and Williams, J.~D.
\newblock 2013.
\newblock {POMDP-based statistical spoken dialog systems: A review}.
\newblock In {\em Proceedings of the IEEE}, volume 101,  pp. 1160--1179.
\newblock IEEE.

\bibitem[\protect\citeauthoryear{Yu \bgroup et al\mbox.\egroup
  }{2017}]{yu2017seqgan}
Yu, L.; Zhang, W.; Wang, J.; and Yu, Y.
\newblock 2017.
\newblock {Seqgan: Sequence generative adversarial nets with policy gradient}.
\newblock In {\em Thirty-First AAAI Conference on Artificial Intelligence}.
\newblock AAAI.

\bibitem[\protect\citeauthoryear{Zhang \bgroup et al\mbox.\egroup
  }{2020}]{zhang2020recent_advances}
Zhang, Z.; Takanobu, R.; Huang, M.; and Zhu, X.
\newblock 2020.
\newblock {Recent Advances and Challenges in Task-oriented Dialog System}.
\newblock {\em Science China Information Sciences}.
\newblock Under Review.

\bibitem[\protect\citeauthoryear{Zhang, Zhao, and
  Yu}{2018}]{zhang2018multimodal}
Zhang, J.; Zhao, T.; and Yu, Z.
\newblock 2018.
\newblock Multimodal hierarchical reinforcement learning policy for
  task-oriented visual dialog.
\newblock {\em ArXiv:1805.03257}.

\bibitem[\protect\citeauthoryear{Zhao and Eskenazi}{2016}]{zhao2016towards}
Zhao, T., and Eskenazi, M.
\newblock 2016.
\newblock Towards end-to-end learning for dialog state tracking and management
  using deep reinforcement learning.
\newblock In {\em Proceedings of the SIGDIAL 2016 Conference},  1--10.
\newblock Los Angeles: Association for Computational Linguistics.

\bibitem[\protect\citeauthoryear{Zhao \bgroup et al\mbox.\egroup
  }{}]{zhaodynamic}
Zhao, Y.; Wang, Z.; Yin, K.; Zhang, R.; Huang, Z.; and Wang, P.
\newblock {Dynamic Reward-based Dueling Deep Dyna-Q: Robust Policy Learning in
  Noisy Environments}.
\newblock In {\em Thirty-Fourth AAAI Conference on Artificial Intelligence}.

\bibitem[\protect\citeauthoryear{Zheng \bgroup et al\mbox.\egroup
  }{2019}]{zheng2019persona}
Zheng, Y.; Chen, G.; Huang, M.; Liu, S.; and Zhu, X.
\newblock 2019.
\newblock Personalized dialogue generation with diversified traits.
\newblock In {\em 3rd Workshop on Conversational AI, NeurIPS}.

\bibitem[\protect\citeauthoryear{Zhou, Arnold, and Yu}{2019}]{zhou2019building}
Zhou, M.; Arnold, J.; and Yu, Z.
\newblock 2019.
\newblock Building task-oriented visual dialog systems through alternative
  optimization between dialog policy and language generation.
\newblock In {\em Proceedings of EMNLP-IJCNLP 2019}.

\bibitem[\protect\citeauthoryear{Zhou \bgroup et al\mbox.\egroup
  }{2017}]{zhou2017end}
Zhou, L.; Small, K.; Rokhlenko, O.; and Elkan, C.
\newblock 2017.
\newblock End-to-end offline goal-oriented dialog policy learning via policy
  gradient.
\newblock In {\em Workshop on Conversational AI, NIPS}.

\bibitem[\protect\citeauthoryear{Zhou \bgroup et al\mbox.\egroup
  }{2020}]{zhou2020design}
Zhou, L.; Gao, J.; Li, D.; and Shum, H.-Y.
\newblock 2020.
\newblock {The Design and Implementation of XiaoIce, an Empathetic Social
  Chatbot}.
\newblock {\em Computational Linguistics} 46(1):53--93.

\end{thebibliography}

